Interactive Perception for Deformable Object Manipulation

Interactive perception enables robots to manipulate the environment and objects to bring them into states that benefit the perception process. Deformable objects pose challenges to this due to significant manipulation difficulty and occlusion in vision-based perception. In this work, we address such a problem with a setup involving both an active camera and an object manipulator. Our approach is based on a sequential decision-making framework and explicitly considers the motion regularity and structure in coupling the camera and manipulator. We contribute a method for constructing and computing a subspace, called Dynamic Active Vision Space (DAVS), for effectively utilizing the regularity in motion exploration. The effectiveness of the framework and approach are validated in both a simulation and a real dual-arm robot setup. Our results confirm the necessity of an active camera and coordinative motion in interactive perception for deformable objects.

==> limitation.tex <==
   \section{Discussion of Limitation}
The implementation of our formulation works for a half-spherical camera action manifold and a loop-shaped SOI, both of which are common for active vision tasks and deformable object features. Other camera action space might require a general manifold representation.
We assume annotated SOI key-points as there exist many reliable key-point detection methods. It is worth to note that our framework does not require a very accurate geometry of SOI, as it is only used for an approximation of a promising subspace. Still, further studies are needed to assess the impact of SOI built from a noisy output of key-point detection models. Concerning failure modes, we observe that the deployed policy can fail at certain camera birth places. These results suggest that DAVS shifts the exploration-exploitation balance in the action search towards more efficient exploitation, improving overall performance at the cost of less exhaustive exploration. This implies that further improvements of the method are needed to ensure complete exploration of the entire action space. Lastly, our experimental results are obtained from physics simulation due to the difficulty of setting up a similar real interactive perception system, and absence of an applicable baseline method. A real robot validation can further demonstrate the effectiveness of the proposed framework in less controlled environments.
